Diving into the Depths of Spotting Text in Multi-Domain Noisy Scenes

When used in a real-world noisy environment, the capacity to generalize to multiple domains is essential for any autonomous scene text spotting system. However, existing state-of-the-art methods employ pretraining and fine-tuning strategies on natural scene datasets, which do not exploit the feature interaction across other complex domains. In this work, we explore and investigate the problem of domain-agnostic scene text spotting, i.e., training a model on multi-domain source data such that it can directly generalize to target domains rather than being specialized for a specific domain or scenario. In this regard, we present the community a text spotting validation benchmark called Under-Water Text (UWT) for noisy underwater scenes to establish an important case study. Moreover, we also design an efficient super-resolution based end-to-end transformer baseline called DA-TextSpotter which achieves comparable or superior performance over existing text spotting architectures for both regular and arbitrary-shaped scene text spotting benchmarks in terms of both accuracy and model efficiency. The dataset, code and pre-trained models will be released upon acceptance.

==> tex/supply.tex <==

% \documentclass[10pt,twocolumn,letterpaper]{article}

% \usepackage{iccv}
% \usepackage{times}
% \usepackage{epsfig}
% \usepackage{graphicx}
% \usepackage{adjustbox}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% \usepackage{dsfont}
% \newcommand{\cmark}{\ding{51}} %
% \newcommand{\xmark}{\ding{55}} %
% \usepackage{pifont}

% Include other packages here, before hyperref.

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
% \usepackage[pagebackref=true,breaklinks=true,colorlinks,bookmarks=false]{hyperref}
% \def\iccvPaperID{11859} % *** Enter the ICCV Paper ID here
% \def\httilde{\mbox{\tt\raisebox{-.5ex}{\symbol{126}}}}

% % Pages are numbered in submission mode, and unnumbered in camera-ready
% \ificcvfinal\pagestyle{empty}\fi

% \begin{document}

%%%%%%%%% TITLE
% \title{MixupTextSpotter: Towards Domain Generalized Scene Text Spotting}
% \title{DG-TextSpotter: Towards Domain Generalized Scene Text Spotting with Faster Self-Attention Supplementary Material}

% \author{Alloy Das\\
% Indian Statistical Institute\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \maketitle
% % Remove page # from the first page of camera-ready.
% \ificcvfinal\thispagestyle{empty}\fi



\paragraph{Datasets} 
The following datasets have been used to train and evaluate the performance of DG-TextSpotter.\\

\noindent
\textit{ICDAR 2015}~\cite{karatzas2015icdar} is the official dataset for ICDAR 2015 robust reading competition for regular text spotting. It has 1000 training and 500 testing images. \\
\noindent
\textit{Total-text}~\cite{ch2020total} is a well-known arbitrary-shaped text spotting benchmark with 1255 training and 300 testing images. The text instances in this benchmark are at the word level.\\ 
\noindent
\textit{CTW1500}~\cite{liu2019curved} is another arbitrary-shaped text spotting benchmark consisting of 1000 training and 500 testing images. The text instances in this benchmark are at the multi-word level.\\
\noindent
\textit{Vintext}~\cite{nguyen2021dictionary} is a recently Vietnamese text dataset. It
consists of 1200 training images and 500 testing images.\\
\noindent
\textit{SynthText 150k} dataset synthesized in~\cite{liu2020abcnet}, consisting of 94723 images with mostly straight text and 54327 images with major curved text. \\
\noindent
\textit{ICDAR 2017 MLT}~\cite{nayef2017icdar2017} is a multi-lingual text dataset. It contains 7200 training images and 1800 validation images. We only select the images containing English texts for training.


% \begin{figure}
%     \centering
%     \includegraphics[width = 0.48\textwidth]{supply_images/Screenshot 2023-03-06 at 19-37-07 TensorBoard.png}
%     \caption{\textbf{Trade-off between text spotting performance h-mean vs number of training iterations}: The blue curve indicates the model without the SAC2 attention module while the  orange curve depicts the model performance with our proposed SAC2 module.}
%     \label{fig:Conver}
% \end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{layers_images/res_layers.png}
    \caption{\textbf{Visualization of attention maps for Resnet-50 feature backbone}. (L) to (R) shows attention maps starting from the first layer.}
    \vspace{-0.302cm}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width = \textwidth]{layers_images/swin_layers.png}
    \caption{\textbf{Visualization of attention maps for Swin-Tiny feature backbone}. (L) to (R) shows attention maps from the first layer.}
\end{figure*}

\begin{figure*}[ht]
\centering
\begin{tabular}{c c c } 
\includegraphics[height=4cm, width= 4cm]{compare/abcnet_1.jpg}&
\includegraphics[height=4cm, width= 4cm]{compare/abcnet v2_.jpg}&
\includegraphics[height=4cm, width= 4cm]{compare/mango_1.jpg}\\
\includegraphics[height=4cm, width= 4cm]{compare/abcnet_crop.jpeg}&
\includegraphics[height=4cm, width= 4cm]{compare/abc v2_crop.jpeg}&
\includegraphics[height=4cm, width= 4cm]{compare/mango_crop.jpeg}\\
(a) ABCNet &(b) ABCNetv2 &(c) MANGO \\
\includegraphics[height=4cm, width= 4cm]{compare/swin_1.jpg}&
\includegraphics[height=4cm, width= 4cm]{compare/testr_1.jpg}&
\includegraphics[height=4cm, width= 4cm]{compare/my_1.jpg}\\
% \includegraphics[height=4cm, width= 4cm]{compare/swin_crop.png}&
% \includegraphics[height=4cm, width= 4cm]{compare/testr_crop.png}&
% \includegraphics[height=4cm, width= 4cm]{compare/my_crop.png}\\
\includegraphics[height=4cm, width= 4cm]{compare/swin_crop1.png}&
\includegraphics[height=4cm, width= 4cm]{compare/testr_crop1.png}&
\includegraphics[height=4cm, width= 4cm]{compare/my_crop1.png}\\
(d) SwinTextSpotter &(e) TESTR & (f) \textbf{DG-TextSpotter}\\
\end{tabular}
\caption{\textbf{Qualitative comparison with SOTA approaches}: The above figure shows a sample test image from the TotalText dataset and shows the end-to-end text spotting performance of DG-TextSpotter when compared to existing SOTA methods. We show a more fine-grained comparison with all the competitors.}
\label{fig:figsotacom}
\end{figure*}

\paragraph{Evaluation Metrics} The standard metrics Recall (R), Precision (P), and F-measure (F) have been used for evaluating text detection performance. While the end-to-end performance evaluations of text recognition use the None (without using lexica) and Full (using lexica) settings. Furthermore, the Strong (S), Weak (W), and Generic (G) lexica settings have been used to measure recognition performance. For all images, the S, W, and G settings correspond to a small lexicon with 100 words, a lexicon with all the words in the test set, and a lexicon with 90,000 words, respectively. By varying the lexicon sizes, we test the recognition performance under different settings. The proposed system has been evaluated against the state-of-the-art using standard evaluation protocols used in these datasets, which are based on calculating IoU between the predicted and ground-truth polygons. 




\section{Further Discussions and Insights}

\paragraph{More Experiments on Encoder and Decoder } We have performed some experiments on the possible combinations of the number of decoder and encoder layers to show the trade-off between the choice of the number of encoder/decoder layers with detection and end-to-end performance. All the results are illustrated in Table \ref{tab:my-table10}. The experiments are performed on the Total-Text dataset in the fine-tuning configuration. We observe that with the uniform number of layers (6) for the encoder and decoder blocks, we achieve the most optimal performance for both detection and end-to-end spotting.


\begin{table}[h]
\centering
\caption{Experiments on the number of Encoder and Decoder layers.}
\begin{tabular}{@{}cccccc@{}}
\toprule
 \multicolumn{2}{c}{No of Layers} & \multicolumn{3}{c}{Detection} & End-to-end \\\cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-6}
Encoder&Decoder& P & R & F &   None \\ \hline
4 & 6  & \textbf{90.85}     & 74.03  & 81.58  &  59.80  \\
6 & 4  & 90.17     & 72.90  & 80.62  & 59.40  \\
6 & 6  & 88.87    & \textbf{76.47} & \textbf{82.20} & \textbf{60.06 } \\
\bottomrule
\end{tabular}

\label{tab:my-table10}
\end{table}


\paragraph{Performance Trade-off during Training}  

As depicted in Fig.~\ref{fig:Conver},  we observe the effectiveness of the SAC2 attention module introduced in the model (as shown in orange curve) when compared to the one with normal deformable attention~\cite{zhu2020deformable}. The key explanation behind this phenomenon is the usage of cyclic convolutions which was previously proposed for real-time instance segmentation~\cite{peng2020deep} for efficient feature learning. Using this layer on top of the self-attention module along with the reference point resampling strategy used for both position and character queries helps in faster convergence during training and a better end-to-end spotting h-mean.   



\paragraph{How does DG-TextSpotter fare qualitatively when compared to other approaches?} As shown in Fig.~\ref{fig:figsotacom}, we show an example test case from TotalText~\cite{ch2020total} and analyse how our method fares compared to other competitors. We realise that DG-TextSpotter is the only method which could spot the apostrophe (') special character in the word "Let's". Also it spots the words in a case-sensitive manner, contrary to SwinTextSpotter~\cite{huang2022swintextspotter} which is our closest competitor. Also, the high confidence scores of the spotted text predictions in our model when compared to other approaches like ABCNet series~\cite{liu2020abcnet, liu2021abcnet} or MANGO~\cite{qiao2021mango} are also very noticeable. This also justifies the superiority of the quantitative performance of our model when compared to others.     

\paragraph{To what extent does Swin-Tiny feature backbone benefit DG-TextSpotter?} We show a comparison of attention maps visualized in different layers for ResNet-50 backbone~\cite{he2016deep} when compared to the Swin-Tiny~\cite{liu2021swin} variant. The Swin attention better captures the global interactions between the different objects to localize the text region which helps them to get a substantial gain over ResNet-50 which primarily captures more local spatial relationships with the attention. The hierarchical shifted-window-based mechanism is highly useful to control the attention on top of the text region boundaries to have a more complete understanding using better contextual cues.    

\paragraph{Qualitative Performance Analysis on CTW1500} As shown in Fig.~\ref{fig:figsupctw}, CTW1500 is a challenging benchmark when it comes to spotting arbitrary-shaped text at the sentence level. Examples (f) and (h) show how DG-TextSpotter is able to spot multiple words together correctly even though it's primarily pre-trained on word-level datasets.   

\paragraph{Qualitative Performance Analysis on Total-Text} As shown in Fig.~\ref{fig:figsuptt}, TotalText is an arbitrary-shaped text spotting dataset at the word-level. The examples show the complexity of different scene conditions to spot text, where DG-TextSpotter performs comprehensively well. Examples (a),(f) and (i) exclusively show images with lots of noises that it's hard to detect and on top recognise the text. DG-TextSpotter is robust and adapts itself to spot text in such complex scenes.  

\paragraph{Qualitative Insights on Low-Resource Vintext} As shown in Fig.~\ref{fig:figsupvin}, VinText is a relatively new benchmark proposed in ~\cite{nguyen2021dictionary} where its a challenging script containing more number lexicons than English which makes it difficult for vision-based Text Spotting~\cite{liu2020abcnet,liao2020mask} models to fare well and there is a need for a dictionary-guided algorithm as shown in ~\cite{nguyen2021dictionary}to improve the spotting results. DG-TextSpotter improvises on the text-spotting backbone to achieve state-of-the-art performance using no dictionary-guided text supervision, surpassing the nearest competitor~\cite{huang2022swintextspotter}. The results show that even the special characters in Vietnamese script are well recognised without any guided text supervision. 

\paragraph{Qualitative Insights on Regular Text ICDAR 2015} As shown in Fig.~\ref{fig:figsupic15}, the DG-TextSpotter framework is robust to spot even regular text and achieve superior performance. ICDAR-15 is a challenging benchmark as the examples in Fig.~\ref{fig:figsupic15} especially (e),(f), (g), (l) which do not have focused scene text and are highly challenging to spot them. DG-TextSpotter achieves state-of-the-art results even in this benchmark and the aforementioned qualitative results justify them. 

\paragraph{Scope for Improvement} As shown in Fig.~\ref{fig:figfail}, we observe a couple of failure cases taken from all the 4 evaluation benchmarks~\cite{ch2020total,karatzas2015icdar,nguyen2021dictionary, liu2019curved}. Results depict there is still scope for improvement in these scenarios especially when the text is not focused and the scene complexity is even higher. 


% \paragraph{Comparison of Different Layers of Resnet-50 and Swin Backbone.}






% \begin{table}[ht]
% \centering
% \caption{Domain Generalization Experiments}
% \begin{adjustbox}{max width=.48\textwidth}
% \begin{tabular}{ccccc}
% \toprule
% \multirow{2}{*}{Dataset}& \multirow{2}{*}{Method}& \multicolumn{3}{c}{Detection} \\  \cmidrule(lr){3-5}
% & & P& R & F \\ \hline
% \multirow{2}{*}{Total-Text}& Pretrained with Eng SynthText  & -&-& -\\
% & Previous + RECTS &-&-&-\\ \hline
% % & Previous + ICDAR15 &-&-&-\\ 
% % & Previous + Total-Text &-&-&-\\ \hline
% \multirow{2}{*}{ICDAR2015}& Pretrained with Eng SynthText  & -&-& -\\
% & Previous + RECTS&-&-&-\\ \hline
% % & Previous + Total-Text &-&-&-\\ 
% % & Previous + ICDAR15 &-&-&-\\ \hline
% \multirow{2}{*}{CTW1500}& Pretrained with Eng SynthText  & -&-& -\\
% & Previous + RECTS&-&-&-\\ \hline
% % & Previous + ICDAR15 &-&-&-\\ 
% % & Previous + Total-Text &-&-&-\\ 
% % & Previous + CTW1500 &-&-&-\\
% \multirow{2}{*}{RECTS}& Pretrained with Chi SynthText  & -&-& -\\
% & Previous + MLT&-&-&-\\ 
% \bottomrule
% \end{tabular}
% \end{adjustbox}

% \label{tab:my-table9}
% \end{table}



% \paragraph{Comparison with State of the art Methods and DG-TextSpotter.}












% \section{Some Qualitative Examples on CTW1500 Dataset.}


\begin{figure*}[ht]
\centering
\begin{tabular}{c c c c} 
\includegraphics[height=4cm, width= 4cm]{supply_images/1006.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1008.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1010.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1012.jpg}\\
(a)&(b)&(c)&(d)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/1016.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1018.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1019.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1021.jpg}\\
(e)&(f)&(g)&(h)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/1022.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1025.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1049.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/1050.jpg}\\
(i)&(j)&(k)&(l)\\
\end{tabular}
\caption{\textbf{Performance Analysis on CTW1500.} Some qualitative test cases of our method on images from CTW1500.}
\label{fig:figsupctw}
\end{figure*}



% \section{Some Qualitative Examples on Total-Text Dataset.}
\begin{figure*}[ht]
\centering
\begin{tabular}{cccc} 
\includegraphics[height=4cm, width= 4cm]{supply_images/0000001.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000002.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000020.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000036.jpg}\\
(a)&(b)&(c)&(d)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/0000041.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000042.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000047.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000056.jpg}\\
(e)&(f)&(g)&(h)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/0000060.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000061.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000064.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/0000065.jpg}\\
(i)&(j)&(k)&(l)\\
\end{tabular}
\caption{\textbf{Performance Analysis on TotalText.} Some qualitative test cases of our method on images from TotalText.}
\label{fig:figsuptt}
\end{figure*}



% \section{Some Qualitative Examples on Vintext Dataset.}
\begin{figure*}[ht]
\centering
\begin{tabular}{cccc} 
\includegraphics[height=4cm, width= 4cm]{supply_images/im1536.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1537.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1539.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1542.jpg}\\
(a)&(b)&(c)&(d)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/im1545.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1559.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1565.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1577.jpg}\\
(e)&(f)&(g)&(h)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/im1588.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1599.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1604.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/im1612.jpg}\\
(i)&(j)&(k)&(l)\\
\end{tabular}
\caption{\textbf{Performance Analysis on Low Resource VinText.} Some qualitative test cases of our method on images from the Vietnamese Text dataset.}
\label{fig:figsupvin}
\end{figure*}




% \section{Some Qualitative Examples on ICDAR 2015 Dataset.}
\begin{figure*}[ht]
\centering
\begin{tabular}{cccc} 
\includegraphics[height=4cm, width= 4cm]{supply_images/img_5.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_10.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_14.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_25.jpg}\\
(a)&(b)&(c)&(d)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/img_31.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_52.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_57.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_90.jpg}\\
(e)&(f)&(g)&(h)\\
\includegraphics[height=4cm, width= 4cm]{supply_images/img_108.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_125.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_149.jpg}&
\includegraphics[height=4cm, width= 4cm]{supply_images/img_299.jpg}\\
(i)&(j)&(k)&(l)\\
\end{tabular}
\caption{\textbf{Performance Analysis on ICDAR15.} Some qualitative test cases of our method on images from ICDAR15.}
\label{fig:figsupic15}
\end{figure*}


% \section{Some Failure Cases of DG-TextSpotter.}

\begin{figure*}[ht]
\centering
\begin{tabular}{c c c c} 
\includegraphics[height=4cm, width= 4cm]{failure/0000048.jpg}&
\includegraphics[height=4cm, width= 4cm]{failure/img_6.jpg}&
\includegraphics[height=4cm, width= 4cm]{failure/im1507.jpg}&
\includegraphics[height=4cm, width= 4cm]{failure/1024.jpg}\\
(a)&(b)&(c)&(d)\\
\includegraphics[height=4cm, width= 4cm]{failure/0000058.jpg}&
\includegraphics[height=4cm, width= 4cm]{failure/img_7.jpg}&
\includegraphics[height=4cm, width= 4cm]{failure/im1516.jpg}&
\includegraphics[height=4cm, width= 4cm]{failure/1009.jpg}\\
(e)&(f)&(g)&(h)\\
\end{tabular}
\caption{\textbf{Failure Cases.} Illustration of some failure cases of our method a and e from Total Text, b and f are from ICDAR15, c and g are from Vintext and d and h from CTW1500 dataset.}
\label{fig:figfail}
\end{figure*}


{\small
\bibliographystyle{ieee_fullname}
\bibliography{egbib}
}

\end{document}
